Physics Performance Report for PANDA: Strong Interaction Studies with Antiprotons

To study fundamental questions of hadron and nuclear physics in interactions of antiprotons with nucleons and nuclei, the universal PANDA detector will be built. Gluonic excitations, the physics of strange and charm quarks and nucleon structure studies will be performed with unprecedented accuracy thereby allowing high-precision tests of the strong interaction. The proposed PANDA detector is a state-of-the art internal target detector at the HESR at FAIR allowing the detection and identification of neutral and charged particles generated within the relevant angular and energy range. This report presents a summary of the physics accessible at PANDA and what performance can be expected.

==> panda_pb_rev.tex <==
Revision: 810


==> phys/exotic/phys_exo_summary.tex <==
% FILE: phys_exo_summary.tex
%
\subsubsection{Summary}
%
\COM{Author(s): K. Peters}
\COM{Referee(s): F. Iazzi}
%
From the simulation of the benchmark channels we can draw the conclusion that...
%
% EOF: phys_exo_summary.tex

==> sty/panda_commands.tex <==
% def_panda_cmd.tex
%
\RequirePackage[centertags]{amsmath}
%
\RequirePackage{xspace}
%\RequirePackage{ulem}
%
%\def\MARK#1{\texorpdfstring{{\emph{\textcolor{red}{#1}}}}{{#1}}}
%\def\MARK#1{\emph{\textcolor{red}{#1}}}
%\def\MARK#1{{\bf \textcolor{red}{#1}}}
\def\MARK#1{{#1}}
% use to mark text 
% (Text will be kept, but the marking removed in the final document)
%
%\def\COM#1{\fbox{\parbox{\swidth}{\textcolor{red}{\bf COMMENT: #1}}}}
\def\COM#1{}
% use to add comments
% (The whole will be removed in the final version)
%
% use to mark parts, which shouldn't be present in the cost-free version

\def\OnlyLayoutColumnBreak{{\vfill\newpage}}%

\def\OnlyLayoutPageBreak{{\vfill\clearpage}}%

\def\OnlyLayoutDoublePageBreak{{\vfill\cleardoublepage}}%

%
\def\bfg{\begin{figure}}%
\def\efg{\end{figure}}%
\def\bc{\begin{center}}%
\def\ec{\end{center}}%
\def\bi{\begin{itemize}}%
\def\ei{\end{itemize}}%
\def\beq{\begin{equation}}%
\def\eeq{\end{equation}}%
\def\bn{\begin{eqnarray}}%
\def\en{\end{eqnarray}}%
\def\ba#1{\left(\begin{array}{#1}}%
\def\ea{\end{array}\right)}%
\def\bef{\begin{equation}\fbox{$\displaystyle}%
\def\eef{$}\end{equation}}%
\def\bnf{\bef\ba{rcl}}%
\def\enf{\ea\eef}%
\newcommand{\beal}{\begin{align}}
\newcommand{\eal}{\end{align}}
\newcommand{\bespl}{\begin{split}}
\newcommand{\espl}{\end{split}}
%\def\refeq#1{\Eqref{#1}\xspace}%
%\def\Refsec#1{sec.~\ref{#1}\xspace}%
%\def\Refchap#1{\Refchap{#1}\xspace}%
%\def\Reffig#1{\Reffig{#1}\xspace}%
%\def\Reftbl#1{\Reftbl{#1}\xspace}%
%\def\reftab#1{\Reftbl{#1}\xspace}%
\def\Refeq#1{Eq.~\ref{#1}\xspace}%
\def\Refeqs#1{Eqs.~\ref{#1}\xspace}%
\def\Refsec#1{Sec.~\ref{#1}\xspace}%
\def\Refchap#1{Chap.~\ref{#1}\xspace}%
\def\Reffig#1{Fig.~\ref{#1}\xspace}%
\def\Reffigs#1{Figs.~\ref{#1}\xspace}%
\def\Reftbl#1{Table~\ref{#1}\xspace}%
\def\Reftbls#1{Tables~\ref{#1}\xspace}%
\def\RefeqX#1{Eq.~\ref{#1}}%
\def\RefeqsX#1{Eqs.~\ref{#1}}%
\def\RefsecX#1{Sec.~\ref{#1}}%
\def\RefchapX#1{Chap.~\ref{#1}}%
\def\ReffigX#1{Fig.~\ref{#1}}%
\def\ReffigsX#1{Figs.~\ref{#1}}%
\def\ReftblX#1{Table~\ref{#1}}%
\def\ReftblsX#1{Tables~\ref{#1}}%
%\def\Reftab#1{Table~\ref{#1}\xspace}%
\def\ub{\underbrace}%
%
\def\vps{\hspace*{5mm}}%
\def\dsty{\displaystyle}%
%
\newcounter{auth}%
\setcounter{auth}{0}%
\def\authitem#1{\addtocounter{auth}{1}#1}%
\def\authitemi#1#2{\addtocounter{auth}{1}#2$^{#1}$}%
\newcounter{inst}%
\setcounter{inst}{0}%
\def\institem#1{\par \addtocounter{inst}{1}#1\\}%
\def\lastitem{\ }%
\def\respitem#1{\institem{{\bf #1}\lastitem\\}}%
\let\groupitem=\authitem
%
\newcommand{\captionfonts}{\small}
%
\makeatletter  % Allow the use of @ in command names
\long\def\@makecaption#1#2{%
  \vskip\abovecaptionskip
  \sbox\@tempboxa{{\captionfonts {\bf #1:} #2}}%
  \ifdim \wd\@tempboxa >\hsize
    {\captionfonts {\bf #1:} #2\par}
  \else
    \hbox to\hsize{\hfil\box\@tempboxa\hfil}%
  \fi
  \vskip\belowcaptionskip}
\makeatother   % Cancel the effect of \makeatletter
%
% a few commands to change the figure placing (commented are the default values)
%\renewcommand{\textfraction}{0.1} % 0.2
%\renewcommand{\bottomfraction}{0.4} % 0.3
%\renewcommand{\dbltopfraction}{0.8} % 0.7
%\renewcommand{\dblfloatpagefraction}{0.3} % 0.5
%\renewcommand{\floatpagefraction}{0.3} % 0.5
%\setcounter{dbltopnumber}{3} % 2
%\setcounter{bottomnumber}{2} % 1
%
\def\markpanda#1#2{\markboth{\Panda{} - #1}{FAIR/PANDA/#2}}%
%
% EOF: def_panda_cmd.tex


==> sty/panda_detector.tex <==
% panda_detector.tex
%
\RequirePackage{xspace}
%
\def\INST#1{\texorpdfstring{{\sffamily #1}}{{#1}}\xspace}%
%
\def\PANDA{\texorpdfstring{$\overline{\mbox{\sffamily P}}${\sffamily ANDA}}{Panda}\xspace}%
\def\Panda{\texorpdfstring{$\overline{\mbox{\sffamily P}}${\sffamily ANDA}}{Panda}\xspace}%
\def\panda{\texorpdfstring{$\overline{\mbox{\sffamily P}}${\sffamily ANDA}}{Panda}\xspace}%
\def\HESR{\INST{HESR}}%
\def\Hesr{\INST{HESR}}%
\def\GSI{\INST{GSI}}%
\def\Gsi{\INST{GSI}}%
\def\FAIR{\INST{FAIR}}%
\def\Fair{\INST{FAIR}}%
%
% General definitions
%
\def\Ts{TS\xspace}
\def\Fs{FS\xspace}
\def\Mvd{MVD\xspace}
\def\Emc{EMC\xspace}
\def\TsEmc{TS-EMC\xspace}
\def\FsEmc{FS-EMC\xspace}
\def\Had{HAD\xspace}
\def\Muo{MUO\xspace}
\def\TsMuo{TS-MUO\xspace}
\def\FsMuo{FS-MUO\xspace}
\def\Stt{STT\xspace}
\def\Tpc{TPC\xspace}
\def\Dirc{DIRC\xspace}
\def\Rich{RICH\xspace}
\def\Mdc{MDC\xspace}
\def\TsMdc{TS-MDC\xspace}
\def\FsMdc{FS-MDC\xspace}
\def\Tof{TOF\xspace}
\def\Lum{LUM\xspace}
\def\Mag{MAG\xspace}
\def\TsMag{SOL\xspace}
\def\FsMag{DIP\xspace}
%
% EMC definitions
%
\def\BEMC{barrel EMC\xspace}
\def\FWEMC{forward endcap EMC\xspace}
\def\BWEMC{backward endcap EMC\xspace}
\def\TSEMC{target spectrometer EMC\xspace}
\def\FSEMC{forward spectrometer EMC\xspace}
\def\TsEmc{\TSEMC}
\def\FsEmc{\FSEMC}
%
\def\LAAPD{LAAPD\xspace}
\def\LAAPDs{LAAPDs\xspace}
\def\VPT{VPT\xspace}
\def\VPTs{VPTs\xspace}
\def\PWOII{PWO-II\xspace}
\def\PWO{PWO\xspace}

% EOF: def_panda_det.tex


==> sty/panda_symbols.tex <==
% def_panda_sym.tex
%
\input{./sty/pennames.sty}
\input{./sty/myunits.sty}
\input{./sty/mymath.sty}
%
\RequirePackage{xspace}
% Upright mu for micro
\DeclareFontFamily{U}{euc}{}% I chose euc because the chart is called Euler cursive
\DeclareFontShape{U}{euc}{m}{n}{<-6>eurm5<6-8>eurm7<8->eurm10}{}%
\DeclareSymbolFont{AMSc}{U}{euc}{m}{n} % I chose AMSc because AMSa and AMSb are defined in the amsfonts-package
\DeclareMathSymbol{\umu}{\mathord}{AMSc}{"16}
%
\def\degrees{\ensuremath{^\circ}\xspace}%
\def\percent{$\,$\%\xspace}%
\def\prm{\ensuremath{^\prime}}%
\def\etc{{\em etc.}\xspace}%
%
% theory stuff
%
\newcommand{\MZ}{M^{\!\!\!\!\!^o}}
\newcommand{\aslash}{\FMslash a}
\newcommand{\Partialslash}{\FMslash \partial}
\newcommand{\vslash}{\FMslash v}
\newcommand{\pslash}{\FMslash p}
\newcommand{\wslash}{\FMslash w}
\newcommand{\lslash}{\FMslash l}
\newcommand{\Lslash}{\FMslash L}
\newcommand{\qslash}{\FMslash q}
\newcommand{\Qslash}{\FMslash Q}
\newcommand{\Pslash}{\FMslash P}
\newcommand{\Wslash}{\FMslash W}
\newcommand{\kslash}{\FMslash k}
\newcommand{\Kslash}{\FMslash K}
\newcommand{\barKslash}{\FMslash {\bar K}}
\newcommand{\barPslash}{\FMslash {\bar P}}
\newcommand{\kapslash }{\FMslash \kappa }
\newcommand{\chiral}[1]{\stackrel{\circ}{#1}}
\def\Re{{\rm Re\,}}
\def\Im{{\rm Im\,}}
\def\prt{\partial}
%
\def\BW{\ensuremath{\mbox{\it BW}}\xspace}%
\def\BR{\ensuremath{\mathcal{B}}\xspace}%
\def\LH{\ensuremath{\mathcal{L}}\xspace}%
\def\CL{\ensuremath{\mbox{\it CL}}\xspace}%
%
\def\vloo{\mbox{\tt VeryLoose}\xspace}
\def\loo{\mbox{\tt Loose}\xspace}
\def\tig{\mbox{\tt Tight}\xspace}
\def\vtig{\mbox{\tt VeryTight}\xspace}
%
\def\tm{\texttrademark}
\def\tmr{\ensuremath{^{\textregistered}}}
%
\def\ppbar{\ensuremath{\mbox{p}\overline{\mbox{p}}}\xspace}%
\def\pbarp{\ensuremath{\overline{\mbox{p}}\mbox{p}}\xspace}%
\def\NNbar{\ensuremath{N\overline{N}}\xspace}%
\def\pbard{\ensuremath{\overline{\mbox{p}}\mbox{d}}\xspace}%
\def\pbarA{\ensuremath{\overline{\mbox{p}}\mbox{A}}\xspace}%
\def\pbarN{\ensuremath{\overline{\mbox{p}}\mbox{N}}\xspace}%
\def\pbard{\ensuremath{\overline{\mbox{p}}\mbox{d}}\xspace}%
\def\pbar{\ensuremath{\overline{\mbox{p}}}\xspace}%s
\def\nbar{\ensuremath{\overline{\mbox{n}}}\xspace}%
\def\pbarn{\ensuremath{\overline{\mbox{p}}\mbox{n}}\xspace}%
\def\nbarn{\ensuremath{\overline{\mbox{n}}\mbox{n}}\xspace}%
\def\NbarN{\ensuremath{\overline{N}N}\xspace}%
%
\def\qbar{\ensuremath{\overline{q}}\xspace}%
\def\cbar{\ensuremath{\overline{c}}\xspace}%
\def\ccbar{\ensuremath{c\overline{c}}\xspace}%
\def\ccbarg{\ensuremath{c\overline{c}g}\xspace}%
\def\cqbar{\ensuremath{c\overline{q}}\xspace}%
\def\cbarq{\ensuremath{\overline{c}q}\xspace}%
\def\uubar{\ensuremath{u\overline{u}}\xspace}%
\def\ddbar{\ensuremath{d\overline{d}}\xspace}%
\def\ssbar{\ensuremath{s\overline{s}}\xspace}%
\def\bbbar{\ensuremath{b\overline{b}}\xspace}%
\def\bqbar{\ensuremath{b\overline{q}}\xspace}%
\def\bbarq{\ensuremath{\overline{b}q}\xspace}%
\def\qqbar{\ensuremath{q\overline{q}}\xspace}%
\def\qqbarg{\ensuremath{q\overline{q}g}\xspace}%
\def\QQbar{\ensuremath{Q\overline{Q}}\xspace}%
%
\def\ee{\ensuremath{e^+e^-}\xspace}%
\def\mumu{\ensuremath{\mu^+\mu^-}\xspace}%
%
\def\piz{\ensuremath{\pi^0}\xspace}%
\def\pip{\ensuremath{\pi^+}\xspace}%
\def\pim{\ensuremath{\pi^-}\xspace}%
\def\pipm{\ensuremath{\pi^\pm}\xspace}%
\def\pimp{\ensuremath{\pi^\mp}\xspace}%
%
\def\K{\ensuremath{K}\xspace}%
\def\Kp{\ensuremath{K^+}\xspace}%
\def\Km{\ensuremath{K^-}\xspace}%
\def\Kpm{\ensuremath{K^\pm}\xspace}%
\def\Kmp{\ensuremath{K^\mp}\xspace}%
\def\KKbar{\ensuremath{K\overline{K}}\xspace}%
\def\Kz{\ensuremath{K^0}\xspace}%
\def\Kbar{\ensuremath{\overline{K}}\xspace}%
\def\Kzbar{\ensuremath{\overline{K}^0}\xspace}%
\def\KzKzbar{\ensuremath{K^0\overline{K^0}}\xspace}%
\def\Ks{\ensuremath{K_S^0}\xspace}%
\def\Kl{\ensuremath{K_L^0}\xspace}%
%
\def\etaprime{\ensuremath{\eta\prm}\xspace}%
\def\pione{\ensuremath{\pi_1}\xspace}%
%
\def\uquark{\ensuremath{u}\xspace}%
\def\dquark{\ensuremath{d}\xspace}%
\def\squark{\ensuremath{s}\xspace}%
\def\cquark{\ensuremath{c}\xspace}%
\def\bquark{\ensuremath{b}\xspace}%
\def\tquark{\ensuremath{t}\xspace}%
%
\def\D{\ensuremath{D}\xspace}%
\def\Dbar{\ensuremath{\overline{D}}\xspace}%
\def\DDbar{\ensuremath{D\overline{D}}\xspace}%
\def\DpDm{\ensuremath{D^+D^-}\xspace}%
\def\Dz{\ensuremath{D^0}\xspace}%
\def\Dzbar{\ensuremath{\overline{D}^0}\xspace}%
\def\DzDzbar{\ensuremath{D^0\overline{D}^0}\xspace}%
\def\DzDzxbar{\ensuremath{D^0\overline{D}^{\ast0}}\xspace}%
\def\Dx{\ensuremath{D^\ast}\xspace}%
\def\Dxbar{\ensuremath{\overline{D}^\ast}\xspace}%
\def\DxDxbar{\ensuremath{D^\ast\overline{D}^\ast}\xspace}%
\def\Dxz{\ensuremath{D^{\ast 0}}\xspace}%
\def\Dxzbar{\ensuremath{\overline{D}^{\ast 0}}\xspace}%
\def\DbarDxx{\ensuremath{D\overline{D}^{\ast\ast}}\xspace}%
%
\def\Ds{\ensuremath{D_s}\xspace}%
\def\Dspm{\ensuremath{D_s^\pm}\xspace}%
\def\Dsmp{\ensuremath{D_s^\mp}\xspace}%
\def\Dsx{\ensuremath{D_s^\ast}\xspace}%
\def\Dsxpm{\ensuremath{D_s^{\ast\pm}}\xspace}%
\def\Dsxmp{\ensuremath{D_s^{\ast\mp}}\xspace}%
\def\DsDsbar{\ensuremath{D_s\overline{D_s}}\xspace}%
\def\DspDsm{\ensuremath{D_s^+D_s^-}\xspace}%
\def\DsxDsxbar{\ensuremath{D_s^\ast\overline{D_s}^\ast}\xspace}%
\def\DsbarDsxx{\ensuremath{\overline{D_s}D_s^{\ast\ast}}\xspace}%
%
\def\jpsi{\ensuremath{J\!/\!\psi}\xspace}%
\def\psiprime{\ensuremath{\psi\prm}\xspace}%
\def\etac{\ensuremath{\eta_c}\xspace}%
\def\etacprime{\ensuremath{\eta\prm_c}\xspace}%
\def\chicJ{\ensuremath{\chi_{cJ}}\xspace}%
\def\chiczero{\ensuremath{\chi_{c0}}\xspace}%
\def\chicone{\ensuremath{\chi_{c1}}\xspace}%
\def\chictwo{{\chi_{c2}}\xspace}%
\def\honec{\ensuremath{h_c}\xspace}%
%
\def\Cascade{\ensuremath{\Xi}\xspace}%
\def\Cascadebar{\ensuremath{\overline{\Xi}}\xspace}%
\def\Lambdabar{\ensuremath{\overline{\Lambda}}\xspace}%
\def\LambdaLambdabar{\ensuremath{\Lambda\overline{\Lambda}}\xspace}%
\def\Omegabar{\ensuremath{\overline{\Omega}}\xspace}%
\def\OmegaOmegabar{\ensuremath{\Omega\overline{\Omega}}\xspace}%
\def\Sigmabar{\ensuremath{\overline{\Sigma}}\xspace}%
\def\SigmaSigmabar{\ensuremath{\Sigma\overline{\Sigma}}\xspace}%
\def\CascadeCascadebar{\ensuremath{\Xi\overline{\Xi}}\xspace}%
\def\Lambdac{\ensuremath{\Lambda_c}\xspace}%
\def\Sigmac{\ensuremath{\Sigma_c}\xspace}%
\def\Omegac{\ensuremath{\Omega_c}\xspace}%
\def\Cascadec{\ensuremath{\Xi_c}\xspace}%
%
\def\kev{{\mbox{keV}}\xspace}%
\def\kevcc{{\mbox{keV}\!/\!\mbox{\em c$^2$}}\xspace}%
\def\mev{{\mbox{MeV}}\xspace}%
\def\mevc{{\mbox{MeV}\!/\!\mbox{\em c}}\xspace}%
\def\mevcc{{\mbox{MeV}\!/\!\mbox{\em c$^2$}}\xspace}%
\def\mevccsq{{\mbox{MeV$^2$}\!/\!\mbox{\em c$^4$}}\xspace}%
\def\gev{{\mbox{GeV}}\xspace}%
\def\gevc{{\mbox{GeV}\!/\!\mbox{\em c}}\xspace}%
\def\gevcsq{{\mbox{GeV$^2$}\!/\!\mbox{\em c$^2$}}\xspace}%
\def\gevcc{{\mbox{GeV}\!/\!\mbox{\em c$^2$}}\xspace}%
\def\gevccsq{{\mbox{GeV$^2$}\!/\!\mbox{\em c$^4$}}\xspace}%
%
\def\aC{{\mbox{aC}}\xspace}%
%
\def\barn{\ensuremath{\rm \,b}\xspace}
\def\barnhyph{\ensuremath{\rm -b}\xspace}
\def\mbarn{\ensuremath{\rm \,mb}\xspace}
\def\mbarnhyph{\ensuremath{\rm -mb}\xspace}
\def\mubarn{\ensuremath{\rm \,\mu b}\xspace}
\def\nb{\ensuremath{\rm \,nb}\xspace}
\def\pb {\ensuremath{\rm \,pb}\xspace}
\def\invpb {\ensuremath{\mbox{\,pb}^{-1}}\xspace}
\def\fb   {\ensuremath{\mbox{\,fb}}\xspace}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}\xspace}
%
\def\JPC{\ensuremath{J^{\!P\!C}}\xspace}%
\def\JPCzeropm{\ensuremath{0^{+-}}\xspace}%
\def\JPCzeropp{\ensuremath{0^{++}}\xspace}%
\def\JPCzeromm{\ensuremath{0^{--}}\xspace}%
\def\JPCzeromp{\ensuremath{0^{-+}}\xspace}%
\def\JPConepm{\ensuremath{1^{+-}}\xspace}%
\def\JPConepp{\ensuremath{1^{++}}\xspace}%
\def\JPConemm{\ensuremath{1^{--}}\xspace}%
\def\JPConemp{\ensuremath{1^{-+}}\xspace}%
\def\JPCtwopm{\ensuremath{2^{+-}}\xspace}%
\def\JPCtwopp{\ensuremath{2^{++}}\xspace}%
\def\JPCtwomm{\ensuremath{2^{--}}\xspace}%
\def\JPCtwomp{\ensuremath{2^{-+}}\xspace}%
%
\def\JPCscalar{\JPCzeropp}%
\def\JPCvector{\JPConemm}%
\def\JPCtensor{\JPCtwopp}%
%
\def\GE {\relax\ifmmode{\rm G_E}%
         \else\ensuremath{{\rm G_E}}\fi}
\def\GM {\relax\ifmmode{\rm G_M}%
         \else\ensuremath{{\rm G_M}}\fi}
\def\Fi {\relax\ifmmode{\rm F_1}%
         \else\ensuremath{{\rm F_1}}\fi}
\def\Fii {\relax\ifmmode{\rm F_2}%
         \else\ensuremath{{\rm F_1}}\fi}
\def\qsq {\relax\ifmmode{\rm q^2}%
         \else\ensuremath{{\rm q^2}}\fi}


%
\def\tO{\,\rightarrow\,}
%
\def\extl{\ensuremath{E_{xtl}}\xspace}
\def\ecl{\ensuremath{E_{cl}}\xspace}
\def\emax{\ensuremath{E_{max}}\xspace}
%
% EOF: def_panda_sym.tex

